Set-Based Models for Cryptocurrency Software

Emin G\"un Sirer once said: It's clear that writing a robust, secure smart contract requires extreme amounts of diligence. It's more similar to writing code for a nuclear power reactor, than to writing loose web code [...] Yet the current Solidity language and underlying EVM seems designed more for the latter. Formal methods (FM) are mathematics-based software development methods aimed at producing "code for a nuclear power reactor". That is, due application of FM can produce bug-free, zero-defect, correct-by-construction, guaranteed, certified software. However, the software industry seldom use FM. One of the main reasons for such a situation is that there exists the perception (which might well be a fact) that FM increase software costs. On the other hand, FM can be partially applied thus producing high-quality software, although not necessarily bug-free. In this paper we outline some FM related techniques whose application the cryptocurrency community should take into consideration because they could bridge the gap between "loose web code" and "code for a nuclear power reactor".

==> create.tex <==
\section{\label{create} \textit{Create1}}
$Create1$ is defined as follows:
\begin{zed}
Create1 \defs CreateCallsCC \land ContractCreation
\end{zed}
where $ContractCreation$ (not shown) specifies a contract creation operation which entails computing the so-called \emph{mutated state}, executing the initialization code and computing the final state. The specification of these operations needs a few pages of formal code. However we show the definition of $CreateCallsCC$ which 

\begin{schema}{CreateCallsCC}
\Xi WorldState; \Delta MachineState; \Xi CallStack \\
s?,o?,a?:ADDR; g?,p?,v?:ETH; i?:PROG; e?:\nat \\
\where
cs \neq \langle \rangle \\
cs~1~pc = create \\
s~1 \leq (acc~(ees~1).Ia).bal \\
(ees~1).Ie < 1024 \\
s? = (ees~1).Ia \\
o? = (ees~1).Io \\
g? = g - g \div 64 \\
p? = (ees~1).Ip \\
v? = s~1 \\
i? = toprog((s(2) \upto s(2) + s(3) - 1) \dres m) \\
e? = (ees~1).Ie + 1 \\
s' = \langle newAddr((ees~1).Ia,(acc~(ees~1).Ia).nonce) \rangle
     \cat tail(tail(tail~s)) \\
i' = M(i,s~2,s~3) \\
out' = \langle \rangle \\
step' = ccbegins \\
m' = m \\
g' = g
\end{schema}

The following function transforms an array of memory cells into a program; it is left underspecified.

\begin{axdef}
toprog: (MADDR \pfun BYTE) \fun PROG
\end{axdef}



